Biological Random Walks: multi-omics integration for disease gene prioritization

Motivation: Over the past decade, network-based approaches have proven useful in identifying disease modules within the human interactome, often providing insights into key mechanisms and guiding the quest for therapeutic targets. This is all the more important, since experimental investigation of potential gene candidates is an expensive task, thus not always a feasible option. On the other hand, many sources of biological information exist beyond the interactome and an important research direction is the design of effective techniques for their integration. Results: In this work, we introduce the Biological Random Walks (BRW) approach for disease gene prioritization in the human interactome. The proposed framework leverages multiple biological sources within an integrated framework. We perform an extensive, comparative study of BRW's performance against well-established baselines. Availability and implementation: All code is publicly available and can be downloaded at \url{https://github.com/LeoM93/BiologicalRandomWalks}. We used publicly available datasets, details on their retrieval and preprocessing are provided in the supplementary material.

==> multi_population_table.tex <==
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab:multi_population_table}
\scriptsize
\begin{tabular}{p{1cm}p{2cm}p{7cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}\toprule
\textbf{Candidate Gene} &\textbf{Gene Names} &\textbf{Role in Breast Cancer**} &\textbf{BRW} &\textbf{DADA} &\textbf{DIAMOnD} &\textbf{RWR} &\textbf{RWR-M} \\\midrule
\textbf{AR} & Androgen Receptor &AR has been considered a useful biomarker in BC, depending on the context of breast cancer sub-types. AR acts as a tumor suppressor in ER + ve breast cancers, serving as a favorable prognostic marker. However, AR functions as a tumor promoter in ER-ve breast cancers, including HER2 + ve and triple-negative (TNBC) breast cancers, serving as a poor prognostic factor. AR has also been shown to be predictive of the potential of response to adjuvant hormonal therapy in ER + ve breast cancers and to neoadjuvant chemotherapy in TNBC. Targeting AR alone or other therapeutic agents provides alternatives to existing therapy for breast cancer. (1) &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &0 \\
\textbf{JUN} &Jun Proto-Oncogene, AP-1 Transcription Factor Subunit &JUN is a biomarker and regulatory gene in BC. In patients with short survival time (< 5 years), the expression of JUN in BC tissue is down-regulated and the risk of recurrence of breast cancer is increased. Furthermore, JUN mediates the functions of some important cytokines in BC, such as IL-34, IL-33, and IL-1$\beta$. (2) &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &0 &0 \\
\textbf{STAT3} &Signal Transducer And Activator Of Transcription 3 &STAT3 is a pro-tumorigenic transcription factor implicated in many independent aspects of tumor biology. Accordingly, highly active STAT3 signaling may be a negative prognostic indicator in BC patients. STAT3 signaling is involved in immune evasion and chemoresistance in BC, and ongoing research in this field is leading to new advances in therapies for advanced, high-grade metastatic disease. (3) &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &0 &0 \\
\textbf{NOTCH1} &Notch Receptor 1 &NOTCH1 promotes cell growth, migration, and invasion in triple negative BC (TNBC)as well as it is in part responsible for maintaining CSC stemness in TNBCs. The specifc inhibition of its signaling has a remarkable inhibitory efect on this cancer subtype, thus increasing the sensitivity of TNBC to chemotherapeutic reagents (4) &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &0 &0 &0 \\
\textbf{JAK2} &Janus Kinase 2 &JAK2 and STAT5 are involved in the proliferation, differentiation, and survival of mammary gland epithelial cells. Dysregulation of JAK2-STAT5 activity leads to mammary gland developmental defects and/or diseases, including breast cancer. (5) &\cellcolor[HTML]{A8A8A8}1 &0 &0 &0 &0 \\
\textbf{HDAC1} &Histone Deacetylase 1 & HDAC1 overexpression is associated with a greater risk of long-term invasive recurrence of ductal carcinoma in situ (6) &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 \\
\textbf{SMAD4} &SMAD Family Member 4 &SMAD4 plays a role as both a tumor suppressor and in the progression of BC cells (7). Which target molecule Smad4 is involved with can decide its function as an oncogenic or tumour suppressor. (8) &\cellcolor[HTML]{A8A8A8}1 &0 &0 &0 &0 \\
\textbf{YAP1} & Yes1 Associated Transcriptional Regulator &Elevated levels of YAP1 transcription factors are reported in luminal A and luminal B, Her2+, and TNBC. YAP1 is also linked to metastasis in BC. (9) &\cellcolor[HTML]{A8A8A8}1 &\cellcolor[HTML]{A8A8A8}1 &0 &0 &0 \\
\textbf{RXRA} &Retinoid X Receptor Alpha &RXRA contributes to tumorigenesis (10) and to the induction of the epithelial-mesenchymal transition of triple-negative advanced breast cancer cells (11). &\cellcolor[HTML]{A8A8A8}1 &0 &\cellcolor[HTML]{A8A8A8}1 &0 &0 \\
\textbf{CHD4} &Chromodomain Helicase DNA Binding Protein 4 &Somatic mutations in CHD4 occur at low frequency in BC (12) &\cellcolor[HTML]{A8A8A8}1 &0 &0 &0 &0 \\
\textbf{CBL} &Cbl Proto-Oncogene &CBL is frequently overexpressed in human breast cancer tissues, and the loss of CBL decreases the tumorigenic activity of breast cancer cells in vivo (13) &0 &\cellcolor[HTML]{A8A8A8}1 &0 &0 &\cellcolor[HTML]{A8A8A8}1 \\
\textbf{CLTC} & Clathrin Heavy Chain & &0 &\cellcolor[HTML]{A8A8A8}1 &0 &0 &0 \\
\textbf{DDX5} &DEAD-Box Helicase 5 & &0 &0 &\cellcolor[HTML]{A8A8A8}1 &0 &0 \\
\textbf{HIF1A} &Hypoxia Inducible Factor 1 Subunit Alpha & &0 &0 &\cellcolor[HTML]{A8A8A8}1 &0 &0 \\
\textbf{NCOA1} & Nuclear Receptor Coactivator 1 & &0 &0 &\cellcolor[HTML]{A8A8A8}1 &0 &0 \\
\textbf{JAK3} & & &0 &0 &0 &0 &\cellcolor[HTML]{A8A8A8}1 \\
\textbf{PBRM1} & Polybromo 1 & &0 &0 &0 &0 &\cellcolor[HTML]{A8A8A8}1 \\
\end{tabular}
\end{table}
